Delay Comparison of Delivery and Coding Policies in Data Clusters

A key function of cloud infrastructure is to store and deliver diverse files, e.g., scientific datasets, social network information, videos, etc. In such systems, for the purpose of fast and reliable delivery, files are divided into chunks, replicated or erasure-coded, and disseminated across servers. It is neither known in general how delays scale with the size of a request nor how delays compare under different policies for coding, data dissemination, and delivery. Motivated by these questions, we develop and explore a set of evolution equations as a unified model which captures the above features. These equations allow for both efficient simulation and mathematical analysis of several delivery policies under general statistical assumptions. In particular, we quantify in what sense a workload aware delivery policy performs better than a workload agnostic policy. Under a dynamic or stochastic setting, the sample path comparison of these policies does not hold in general. The comparison is shown to hold under the weaker increasing convex stochastic ordering, still stronger than the comparison of averages. This result further allows us to obtain insightful computable performance bounds. For example, we show that in a system where files are divided into chunks of equal size, replicated or erasure-coded, and disseminated across servers at random, the job delays increase sub-logarithmically in the request size for small and medium-sized files but linearly for large files.

==> Evaluations.tex <==
% !TEX root = ChunksAndQueues.tex

\section{Performance Evaluation}\label{sec:simulations}
Recall that the recursion \eqn{eq:Main_Recursion} allows us to develop efficient simulations without using exponentiality assumptions and event driven Markov chain simulations. 
In this section our goal is to use this recursion to complement our analysis of previous sections by $(a)$ identifying regimes under which our bounds are tight, and $(b)$ developing quantitative understanding of relative performance and scaling laws under $\mathcal{WF}$, $\mathcal{BS}$, and $\mathcal{BR}$. 

We simulate the $\mathcal{WF}$, $\mathcal{BS}$, and $\mathcal{BR}$ polices and empirically compute mean delay for a sequence of systems with increasing number of servers. For each empirical computation, we use $10^5$ sample points. We assume that the chunks are of size $1$ bit each. Further, speed of each server $\mu$ is assumed to be $1$ bits/sec. The load per server $\rho$ is kept fixed at $0.7$ bits per second. 
 The distribution of file-size, \ie, $\pi_k$, is assumed to be $Binomial(p,m)$ where we study plots for various values of $p$; recall that for each value of $p$ this falls within the class of distribution $\Theta(m)$.  

\virag{...........I am assuming two figures for this write up, but please do not feel bound by these or the parameters above; edit as you like.......}

(Figure 1: x-axis -- $m$ varying from 10 to 250, y-axis -- Average delay, $\pi$ is $Binomial(p,m)$, $ p =0.1, 0.3, 0.5, 0.7$, $\mathcal{BR}$ policy, and also included are bounds given by Francois.)  

Figure~1 compares mean-delay under various values of $p$ with the bounds obtained in previous section. We see that the bound is a good approximation of the empirical mean delay for $p \le ...$. Further, observe that the bound as well as empirical delays increase logarithmically in $m$. This can be understood as follows. The binomial distribution concentrates around $pm$, thus most requests for files for a system with large enough $m$ are of size approximately $k= pm$. For such requests, as pointed in previous section, the mean delays are logarithmic in $k$ which is tight when $k$ is large. 

\virag{..........Alternatively, instead of arguing concentration of binomial, if we could produce a simulation which subsamples only those requests with chunk size $\floor{pm}$, we can avoid this heuristic argument involving concentration of the `concave' $\log k$ asymptotic bound. The y-axis would then be average delay over these subsamples. Francois can then provide you with the exact mean delay bound conditioned on $k$.......}

However, when $p$ is very large, for instant $p\ge....$ in the above setting, we see that the increase in mean  is sub-logarithmic. This can be explained as follows. As $p$ increases, the correlation across loads becomes increasingly relevant since an arrival simultaneously loads increasingly larger number of servers. This results into several servers seeing similar loads in steady state. The bound of delays via $\max$ of independent server workloads is conservative in such a scenario. 

(Figure 2: x-axis -- $m$ varying from 10 to 250, y-axis -- average delay, $\pi$ is $Binomial(p,m)$, p =0.1, 0.5, $\mathcal{WF}$, $\mathcal{BS}$, and $\mathcal{BR}$ policies. $\alpha=k+1,k+4$. 

Also $C\log k$ bound given by Francois, and $C^{WF}\log k$, $C^{BS} \log k$ approximations where constants $C^{WF}$ and $C^{WF}$ are obtained heuristically to fit the curves.)

\virag{Btw, if WF is doing more or less same as BS, I am okay in saying it in one line: We observe that performance under BS and WF is more or less the same, hence we focus on BS in this section.}


Figure~2 compares delays under different policies. Note that subject to $\alpha_k=k$, each policy is statistically equivalent. We observe that $WF$ and $BS$ perform significantly better than $BR$ when $\alpha_k > k$.  In fact, the largest gains are achieved when $\alpha_k$ increases from $k$ to $k+1$. This can be explained as follows. The tail of delays have a significant impact on the average.  Allowing even small flexibility in service reduces the tails significantly. This also conforms with the `power of choice' models considered in literature \cite{Mit96,VDK96,YSK15}.   The gains achieved by increasing $\alpha_k$ even further are incremental. 

However, we observe that the delays still increase as $O(\log k)$ in the size of files $k$. However, the constants are now different. Our simulations suggest that for $BS$ and $WF$, the constants reduce by a factor of $...$ and $...$. 












==> lambert.tex <==

This leverages the following two results: 
\begin{theorem} [Theorem 7.4. in \cite{}]
Let $\{ Y_l \}_1 ^\infty $ be a family
of i.i.d $\R _+ $-valued random variables whose common
distribution function $G(\cdot)$ exhibits the tail behavior
$$ P[Y_1 >x]= 1- G(x) = C e^{-qx}( 1 + o(1) ), \quad x \geq 0,$$
for some $q >0$ and $C>0$. Then
$$E \biggl [ \max \bigl \{ Y_1,...,Y_k \bigr \} \biggr ] =
\bigl [ {{\log k}\over {q}} \bigr ]^r \cdot (1+o(1))
$$
with $k$ going to infinity.
\end{theorem}

\begin{lemma}
The steady state $Y$ delay in the M/D/1 queue with arrival rate $\lambda$
and service time $\sigma$, with $\lambda\sigma<1$ has the tail behavior 
$$P[Y >x]= 1- G(x) = C e^{-qx}( 1 + o(1) ), \quad x \geq 0,$$
with
$$
q=\lambda +\frac{W(-\lambda\sigma \exp(-\lambda\sigma)}{\sigma}
$$
where $W$ denotes the principal branch of the Lambert W function.
\end{lemma}

\begin{proof}
The P-K Formula, when applied to the M/D/1 queue, gives 
a steady state delay with a Laplace transform having an
isolated pole at the only solution other than 0 of the equation
$$s=\lambda(1-\exp(-s\sigma)).$$
Elementary calculations show that this solution is precisely
$\lambda +\frac{W(-\lambda\sigma \exp(-\lambda\sigma)}{\sigma}$.
The shape of the tail then follows from classical complex
analysis arguments.
\end{proof}


==> truc.tex <==

\subsection{Proof of Theorem \ref{thm:DelaysViaAssociation}}
We first prove part $(i)$ using induction. Clearly, $W_0$ is associated since all its entries are constant and equal to zero. Suppose $W_n$ is associated for some $n$. We show below that this implies that $W_{n+1}$ is associated as well. 

Recall that under $\mathcal{BR}$ the random vectors $W_n$, $s_n$, and $-\mu\tau_n{\bf 1}$ are mutually independent and are themselves associated. Hence, from part $(ii)$ of Proposition~\ref{prop:AssociationProperties}, we have that the entries of $W_n$, $s_n$, and $-\mu\tau_n{\bf 1}$ are mutually associated. Each entry of $(W_n + c s_n - \mu \tau_{n}  {\bf 1})^+$ is an increasing function of the entries of $W_n$, $s_n$, and $-\mu\tau_n{\bf 1}$. From $m$ applications of part $(i)$ of Proposition~\ref{prop:AssociationProperties},  and then of its part $(iii)$,  we get that $W_{n+1}$ is associated. 

We now prove part $(ii)$ of the theorem. We show that in fact for $\mathcal{BR}$ policy the stochastic dominance is in $\le^{st}$ sense which is stranger than $\le^{icx}$. By definition, the vector $\tilde W_n = (\tilde W_n^i: i=1,\ldots,m)$ is an independent version of $W_n$ for each $n$ under $\mathcal{BR}$ policy. Since $\tilde{s}$ is an independent exchangeable vector, and since both $W_n$ and $\tilde W_n$ are exchangeable, it is sufficient to assume that $\tilde{s}$ is deterministic. Then, the result follows for $\mathcal{BR}$ from Proposition \ref{prop:ComparingMax}. 

For $\mathcal{WF}$ and $\mathcal{BS}$, the result then follows by arguing along the lines of Theorem~\ref{thm:DelayComparision}  while additionally conditioning on $|s_n| = k$. 
\end{proof}


